ROAM: Reinforcement Learning Optimized Adaptive Moving Target Defense for Smart Grid

Smart grids rely on distributed phasor measurement units (PMUs) and wide-area communication networks whose data-acquisition pipelines are vulnerable to stealthy false data injection (FDI) attacks that evade conventional bad-data detection (BDD). Moving target defense (MTD) counters this exposure by continuously remapping sensor identities, but existing schemes apply static or pre-scheduled randomization and are each constrained by a single failure mode: seed-based methods are fast yet fragile to key compromise, while machine learning (ML) based prediction methods are resilient yet incur prohibitive latency. Neither adapts its randomization to live threat evidence. This paper presents ROAM, a deep reinforcement learning (DRL) driven MTD framework in which a deep Q-network (DQN) agent continuously re-optimizes the sensor-to-ID mapping at the aggregation layer. At each decision step, the agent selects the deception coverage, flags the specific sensors to remap, and sets the split of the remapped sensors between seed-based and ML-prediction-based recovery, without modifying PMU hardware and while preserving IEEE C37.118 compatibility. On held-out BDD-compliant FDI scenarios across the IEEE 14-, 57-, and 118- bus systems, ROAM keeps the percentage of stealthy attacks below 3% while sustaining detection rates above 93%. Against an adaptive soft actor-critic (SAC) attacker that observes the defender's configuration, ROAM keeps stealthy attacks below 2.6% with detection above 92%. Hardware-in-the-loop testing on an OPAL-RT platform confirms real-time feasibility, with sub-18ms average shuffle execution and an average reshuffle blind window of 2.6% of the 3-s decision cycle.

==> sections/Introduction.tex <==
\section{Introduction}

% \begin{figure}[!ht]
%     \centering
%     \vspace{-2pt}
%     \includegraphics[width=0.70\columnwidth]{figures/Fig_Hybrid_Remap.pdf}
%     \vspace{-2pt}
%     \caption{Proposed hybrid deception mechanism.}
%     \label{fig:hubridrem}
%     \vspace{-2pt}
% \end{figure}
\IEEEPARstart{A}{dvances} in cyber-physical systems (CPSs) and Internet of Things (IoT) technologies are reshaping critical infrastructure from smart grids and industrial control systems to healthcare and transportation networks. While these platforms deliver unprecedented automation, efficiency, and situational awareness, their interconnected, heterogeneous architectures introduce a substantially larger attack surface, making CPS networks increasingly susceptible to a wide array of cyber threats, including stealthy false data injection (FDI), sensor spoofing, and targeted denial-of-service attacks. The energy sector ranked fourth among the most targeted industries in 2022, accounting for 10.7\% of all cyberattacks~\cite{jenifer}. High-profile incidents such as the Triton/Trisis attack in 2017, which disabled safety systems at a Saudi petrochemical plant, and earlier attacks such as Stuxnet~\cite{stuxnet} and Dragonfly~\cite{Dragonfly} demonstrate the increasing sophistication of cyber threats. These attacks often require deep access to real-time operational data and an intimate understanding of control system architectures. Modern smart grids, particularly components such as energy management systems (EMS) with modules like automatic generation control (AGC), are vulnerable to FDI attacks via communication protocols such as C37.118~\cite{Knesek21SmartGridComm, Vahidi23ICST}, DNP3~\cite{Wlazlo21IET}, and Modbus~\cite{HUITSING200837, Chen15CQR}. Synchrophasor technology, including phasor measurement units (PMUs), has enhanced grid monitoring and control through wide-area measurement systems. However, the distributed and networked nature of PMU-based systems exposes them to cyber threats that target data integrity and system stability~\cite{Sadreazami18SIPN, mohammadi2018attack, Pasqualetti}. Attackers can compromise wide-area networks (WANs) by tricking phasor data concentrators (PDCs) into connecting to spoofed PMUs, thereby gaining access to critical system data or disrupting operations~\cite{Swain24Access}. FDI attacks that manipulate synchrophasor data pose a particular risk to AGC stability~\cite{Jafari22IAS, Jafari23TSG, Saini22NPSC, He21EI2}. These stealthy attacks are engineered to bypass traditional bad-data detectors by exploiting knowledge of the system topology and measurement correlations~\cite{Ran24TII}.


Traditional security measures often fail to protect CPSs due to their static configurations and limited adaptability to evolving threats. To address these challenges, deception-based defense mechanisms have emerged as a promising approach. To counter these vulnerabilities, moving target defense (MTD) has emerged as a proactive cybersecurity paradigm. By continuously altering system configurations, such as manipulating the physical parameters or shifting measurement communication pathways, MTD increases adversarial uncertainty and reduces the exploitation window for attackers attempting man-in-the-middle (MITM) or FDI maneuvers \cite{ZhangTSG23, LakshminarayanaTSG21}. MTD acts as a dynamic shield for power system control, randomizing the attack surface so that any intercepted topology or state information becomes obsolete before an attacker can weaponize it \cite{MohammadpourfardTII25, PagnottaTIFS23, Liu21SmartGridComm, Liu18PESGM}.
Some frameworks such as the deception-defense-based data acquisition framework (DDAF)~\cite{ddaf21} and the intelligent deception-defense-based data acquisition framework (iDDAF)~\cite{iddaf21} leverage randomized sensor ID remapping to obfuscate network topology and mislead adversaries. By transforming stealthy attacks into random data injections, these systems enable effective detection and localization of attack points through outlier analysis. While these solutions have demonstrated high efficacy in experimental settings, their static or predefined randomization strategies may be insufficient against adaptive and persistent adversaries.

Deep reinforcement learning (DRL)-based MTD represents a paradigm shift in proactive security by continuously and unpredictably altering system configurations to deceive attackers. In this work, we extend the principles of deception-based data acquisition by integrating MTD with DRL. Specifically, we propose a deep Q-network (DQN)-driven MTD framework that dynamically orchestrates sensor remapping via both seed-based deterministic and data-driven adaptive reshuffling mechanisms~\cite{iddaf21}. The DQN agent intelligently selects which sensors to shuffle, determines the optimal remapping strategy, and adapts to real-time adversarial activity and system health metrics. Upon observing the system, the framework seamlessly varies the ratio between a computationally efficient, deterministic mapping and a robust, data-driven approach, significantly enhancing resilience against advanced threats. The DQN-driven MTD framework is validated on the IEEE 14, 57, and 118 bus systems and tested in real-time on Opal-RT with PMUs, a custom PDC for real-time aggregation and ID shuffling, and an EMS for state estimation and attack emulation. With optimal parameters, the proposed method performs comparably to the baseline while offering greater robustness against attacks and lower computational overhead.


\section{Related Works}
The exponential growth of sensor networks in critical domains, including smart grids, industrial control systems, and environmental monitoring, has fundamentally transformed the cybersecurity landscape. According to recent threat intelligence reports, CPSs face an unprecedented volume of sophisticated attacks targeting sensor data integrity, with adversaries employing increasingly stealthy techniques to compromise measurement authenticity without triggering traditional detection mechanisms~\cite{Aydeger16LCN}. These attacks can range from simple data manipulation to complex FDI campaigns aimed at misleading control algorithms and destabilizing system operations. MTD has emerged as a promising proactive security paradigm that aims to thwart attacks by continuously changing the attack surface of networked systems~\cite{Eghtesad20Verlag, ref_fdi_agc_rl}. Unlike reactive defenses, MTD strategies proactively adjust system settings, network layouts, and data paths to increase attackers' uncertainty and the difficulty of their attacks. This approach aims to remove the attacker's usual advantage by forcing them to adapt to a constantly shifting environment. Current MTD implementations for sensor networks primarily use two remapping approaches. Seed-based methods employ cryptographically secure pseudo-random generators to deterministically alter sensor IDs and routing paths, offering low overhead and fast reconfiguration. However, they depend on pre-shared keys and synchronized states, making them susceptible to key compromise and desynchronization attacks.~\cite{ddaf21, iddaf21}. In contrast, prediction-based remapping uses machine learning to dynamically generate mappings from historical data and threat patterns, enabling adaptive defense against evolving and unknown attacks. Despite their flexibility, these methods incur higher computational costs and may suffer from accuracy issues in resource-constrained sensor networks~\cite{tan2022wf, hamlet2016dependency}.

The limitations inherent in individual remapping approaches underscore the critical need for a unified defense framework that can intelligently combine the strengths of both methodologies while mitigating their respective weaknesses. Existing implementations lack adaptive switching mechanisms that dynamically select optimal remapping strategies based on real-time threat assessment and system conditions. Furthermore, current approaches lack intelligent orchestration capabilities that can optimize deception parameters, sensor selection criteria, and remapping mode selection to maximize attack detection effectiveness while preserving system performance. Recent advances in DRL have shown significant potential to address complex cybersecurity decision-making problems through autonomous learning and adaptation~\cite{PagnottaTIFS23, Cao24IoT, Kim22TNSM}. DQNs, in particular, have shown remarkable success in environments characterized by high-dimensional state spaces and complex action dependencies~\cite{Chen24NOMS}. The application of DQN-based agents to MTD orchestration presents an opportunity to develop intelligent defense systems that can learn optimal strategies through continuous interaction with dynamic threat environments. 

This work addresses the need for proactive defense against advanced threats by proposing an intelligent hybrid MTD framework that dynamically disrupts measurement correlations to thwart stealthy FDI attacks. Key challenges include designing robust state-action spaces and reward functions, and ensuring convergence in adversarial settings. While conventional reactive methods lag behind adaptive attackers, MTD enhances resilience through system variability. Existing MTD strategies, such as seed-based (efficient but key-dependent) and machine learning-based (adaptive but resource-intensive), present trade-offs. Our DRL-driven hybrid approach unifies these methods, balancing adaptability and efficiency to meet the demands of modern sensor network security. First, it enables dynamic assessment of deception needs based on attack patterns and network conditions, optimizing resource use with minimal performance overhead~\cite{Huang19Verlag, Huang13TPS}. Second, it offers intelligent sensor selection to prioritize protection of critical measurements while preserving system observability~\cite{Rahman14ACM}. Third, it supports adaptive switching between seed-based and prediction-based remapping, guided by real-time synchronization, resource availability, and threat severity.

We propose ROAM, a reinforcement learning optimized adaptive moving target defense, a novel DRL-driven framework designed to enhance the cyber-resilience of smart grid data-acquisition systems. The ROAM architecture features an intelligent orchestration layer that dynamically integrates deterministic seed-based shuffling with data-driven adaptive remapping. By monitoring real-time system integrity and adversarial signatures, ROAM continuously optimizes the grid's defensive posture to mitigate stealthy FDI attacks without compromising operational stability. The primary contributions of this work are summarized as follows:


\begin{itemize}
\item A PDC-layer MTD that unifies seed-based and ML-prediction-based ID remapping with a per-sensor mode assignment, requiring no PMU hardware changes and remaining IEEE C37.118 compatible. The hybrid pathway retains accurate state recovery even under full seed compromise, eliminating the single point of failure of prior deception frameworks.

\item A DQN agent that navigates the combinatorial action space (deception amount, sensor subset, remapping mode) under a multi-objective reward trading detection gain against deception cost, latency, and residual attacker accuracy, with PPO as a controlled on-policy baseline.

\item A zero-sum Markov game in which a soft actor-critic attacker, observing the defender's most recent configuration, learns targeted, stealthy injection strategies. This protocol exposes topology-dependent weaknesses (e.g., a 1.8× EDR degradation for DQN on the 57-bus system) that static attack pools cannot reveal.


\item Sim-to-real transfer of the trained policy, without retraining, to an OPAL-RT hardware-in-the-loop testbed (IEEE 118-bus, 19 PMUs), achieving 83.2\% detection against a coordinated multi-PMU FDI campaign with average shuffle execution of 17.97 ms and a reshuffle blind window below 2.6\% of the cycle.

\end{itemize}



% \begin{itemize}
% \item This is the first work to propose a unified framework that intelligently combines machine-learning–based adaptive remapping with the speed and simplicity of deterministic methods via a smart selection mechanism.

% \item A Deep Q-Network (DQN)-based reinforcement learning agent is designed to optimize three key aspects of the MTD strategy in real time: (a) how many sensors to shuffle, (b) which sensors to shuffle, and (c) which strategy to use for the remapping process, all based on current threat levels and system health.

% \item The framework includes an adaptive threat assessment module that automatically switches from lightweight deterministic mapping to more advanced machine learning methods when signs of attack are detected, improving defense against persistent and evolving threats.

% % \item It also introduces a context-aware decoy data system that confuses attackers without affecting normal operations, adding extra layers of deception to strengthen remapping defenses.

% \item The architecture features built-in failover mechanisms to ensure continuous protection, even if the defense logic is targeted, thereby avoiding a single point of failure.

% \item The DQN agent is trained with a multi-goal reward function that balances three priorities: detecting attacks, maintaining system performance stability, and using resources efficiently while ensuring security improvements without incurring extra operational costs.
% \end{itemize}



% \begin{itemize}
%     \item This work is first to propose a unified framework that seamlessly integrates machine learning-based adaptive remapping techniques with the computational efficiency of deterministic methods through intelligent switching mechanisms.
%     \item A novel Deep Q-Network-based RL agent is developed to dynamically optimize three critical aspects of MTD deployment: (a) the number of sensors to shuffle, (b) the selection of specific sensors for remapping, and (c) the choice between deterministic and data-driven remapping modes, all based on real-time adversarial activity and system integrity metrics.
%     \item The framework incorporates an adaptive threat assessment module that enables seamless transitions from computationally efficient deterministic mapping to sophisticated data-driven strategies upon detecting potential compromises, enhancing resilience against advanced persistent threats.
%     \item We introduce context-aware decoy data deployment mechanisms that actively mislead attackers while preserving operational performance, creating multiple layers of deception that compound the effectiveness of remapping strategies.
%     \item The proposed architecture also includes comprehensive failover capabilities that ensure uninterrupted protection even under direct attacks targeting the defense logic itself, maintaining system security without single points of failure.
%     \item The DQN agent is trained with multi-objective reward functions that balance attack detection effectiveness, system performance preservation, and resource utilization efficiency, ensuring that security enhancements do not compromise operational requirements.
% \end{itemize}


%%%%%%%%%%%%%%%

% We have added the role of WAMPAC in inter-area oscillation damping control in Section II \nur{refer the section number, like Section~\ref{sec:inter-pod}}.
%The rest of the paper is organized as follows: In Section~\ref{sec:technical} we have discussed the proposed hybrid MTD atricheture and discusses the technical details of problem formalization. Section~\ref{sec:evaluation} explains the testbed setup, test cases, and evaluation. Section~\ref{sec:discussion} discusses the outcome of this study, possible mitigation approach, limitations, and future endeavors. We have concluded the paper in Section~\ref{sec:conclusion}. 

The remainder of the paper is organized as follows: Section~\ref{sec:technical} presents the proposed hybrid MTD architecture and details the problem formalization. Section~\ref{sec:evaluation} describes the testbed setup, test cases, and evaluation methodology. Finally, Section~\ref{sec:conclusion} concludes the paper.



==> sections/Nomenclature.tex <==
% %\section*{Nomenclature}

% % \begin{table}[h]
% % \begin{left}
% % \begin{tabular}{ l l }
% %  $\mathcal{E}_{fd}$ & Exciter Voltage \\
% %  $\mathcal{I}_{exc}$ & Exciter Current \\
% %  $\mathcal{I}_{load}$ & Load Current\\
% %  $\mathcal{K}_A$ & Amplifier Gain Constant\\
% %  $\mathcal{K}_E$ & Exciter Gain \\
% %  $ \mathcal{K}_p$ & Proportional Gain \\
% %  $ \mathcal{K}_i$ & Integral Gain \\
% %  $\mathcal{K}_{exc}$ & Exciter Gain \\
% %  $\mathcal{Q}$ & Reactive Power \\
% % $\mathcal{R}_{f}$ & Stabilizer Feedback Variable\\
% %   $\mathcal{T}_A$ & Amplifier Time Constant \\
% %   $\mathcal{T}_E$ & Exciter Time Constant \\
% %  $\mathcal{V}_t$ & Terminal Voltage \\
% %  $\mathcal{V}_R$ & Output Voltage of Amplifier\\
% %  $\mathcal{V}_{ref}$ & Reference Voltage of AVR \\
% %  $\Phi$  & Magnetic Flux of Rotor \\
% %  $\theta$ & Power Factor \\
% % \end{tabular}
% % \label{tab1}
% % \end{left}
% % \end{table}

% %%%%%%%%%%%%%%%%Previous Table%%%%%%%%%%%%%%%

% \begin{table}[!t]
% % \centering
% \caption{Modeling Notations}
% \label{tab:modeling-notations}
% %\scriptsize
% \small
% \begin{tabular}{p{2cm} p{1cm}  p{4.5cm}  }
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Type of\\ Notation\end{tabular}}                         & \textbf{Notation} & \textbf{Description} \\ \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{7}{*}{\textbf{General}} 
% & $\mathcal{B}$ & Set of all buses in the system \\ 
% & $\mathcal{B}^{\mathit{PV}}$ & Set of generator buses    \\        
% & $\mathcal{B}^{\mathit{GV}}$ & Set of generator buses with governors  \\
% & $\mathcal{B}^{\mathit{PQ}}$ & Set of load buses \\ 
% & $\mathcal{B}^{S}$           & Slack bus   \\   
% & $\mathcal{G}$               & Set of all generators  \\     
% & $\mathcal{T}^{P, S, T}$       & Set of all timeslots for primary, secondary, and tertiary  controllers' response  \\ 
% & $\mathcal{V}_{wac}$                  & WAMPAC signal for generator \\
% & $\mathcal{Z}$                  & Set of all areas \\
% & b, c                   & indices for  buses \\
% & i, j                   & indices for  areas \\
% \\ \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Bus\\ Measurements\end{tabular}}}        
% & $\delta$                  & Phase angle of bus\\

% & $\mathcal{P}_{\mathit{L}}$ & Load active power  \\ 

% & $\mathcal{V}_{\mathit{t}}$ & Bus voltage  \\ 

% & $\mathcal{F}_{\mathit{t}}$ & Bus Frequency \\
% \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Generators\\ Measurements\end{tabular}}} & 

% $\mathcal{P}_{\mathit{g}}$ & Electrical power of the generator\\ 
% & $\mathcal{P}_{\mathit{m}}$ & Mechanical power of the govornor\\
% & $\mathcal{P}_{\mathit{r}}$ & Reference set point of the generator \\          
% & $\delta$                  & Rotor angle of the generator \\
% & $\omega$              & Angular frequency of the generator \\
% & $\mathcal{V}_{ref}$  & Reference voltage of AVR in generators \\
% & $\mathcal{V}_{pss}$  & Output signal of PSS in generators \\
% & $\mathcal{V}_{avr}$  &  Output signal of the avr in generators \\
% & $\mathcal{V}_{r}$  &  Output signal of the stator in generators \\
% & $\mathcal{E}_{fd}$  &  Induced voltage of stator in generators \\
% \hline 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Fixed \\ Parameters\end{tabular}}}       
% & $\mathcal{R}$                & Droop characteristics of generator \\ 
% & $\Delta T$                       & Discretized time-step size(s)  \\
% & $\mathcal{T}$                & Time-constant of the generator \\                        
% & $\mathcal{B}_{A}$   & Imaginary part of line admittance (siemens)\\
% & $\mathcal{G}_{A}$   & Real part of line admittance (mho) \\
% & $\omega_{s}$              & Reference angular frequency  \\
% & $\mathcal{\delta}_{s}$      & Reference rotor angle of the slack bus  \\
% & $\mathcal{H} $     & Inertia constant of generator\\ 
% & $\mathcal{K}_{P}$     & Proportional constant\\ 
% & $\mathcal{K}_{I}$     & Integral constant \\ 

% & $\mathcal{K}_{D}$     & Derivative constant\\ 


% \hline
% % \multirow{1}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Variable \\ Parameters\end{tabular}}}     
% % & $\mathcal{ACE}^{i}_{t}$ & Area control error of area $i$ at time $t$ (i.e., $i$ $\in$ $\mathcal{Z}$) \\

% % & $\mathcal{ACE}^{b}_{t}$ & Area control error for the generator connected to bus $b$ at time $t$ (i.e., $b$ $\in$ $\mathcal{B}^{\mathit{GV}}$) \\
% % \\ \hline

% \multirow{1}{*}{\textbf{\begin{tabular}[c]{@{}l@{}} BDD \\ Parameter\end{tabular}}}     
% & $\tau_{\omega} $ & BDD threshold for frequency \\

% & $\tau_{wac} $ & BDD threshold of WAMPAC signal\\
% % & $\tau_{tie}^i $ & Bad data detection threshold for tie line power of area i \\
% & $\tau_{v} $ & BDD threshold for voltage \\
% & $\epsilon_{\omega}$ & Slack term for frequency attack at AGC\\ 
% & $\epsilon_{wac}$ & Slack term for frequency attack at WAMPAC\\ 
% & $\epsilon_{v}$ & Slack term for attack on voltage at AVR \\ 
% & $\bar{\tau}_f $ & Over and under frequency threshold \\
% & $\bar{\tau}_{v}$ & Over and under voltage threshold \\ \hline

% \end{tabular}
% % \normalsize
% \end{table}
% %%%%%%%%%%%

